Radio-Optical Galaxy Shape Correlations in the COSMOS Field

We investigate the correlations in galaxy shapes between optical and radio wavelengths using archival observations of the COSMOS field. Cross-correlation studies between different wavebands will become increasingly important for precision cosmology as future large surveys may be dominated by systematic rather than statistical errors. In the case of weak lensing, galaxy shapes must be measured to extraordinary accuracy (shear systematics of $< 0.01\%$) in order to achieve good constraints on dark energy parameters. By using shape information from overlapping surveys in optical and radio bands, robustness to systematics may be significantly improved without loss of constraining power. Here we use HST-ACS optical data, VLA radio data, and extensive simulations to investigate both our ability to make precision measurements of source shapes from realistic radio data, and to constrain the intrinsic astrophysical scatter between the shapes of galaxies as measured in the optical and radio wavebands. By producing a new image from the VLA-COSMOS L-band radio visibility data that is well suited to galaxy shape measurements, we are able to extract precise measurements of galaxy position angles. Comparing to corresponding measurements from the HST optical image, we set a lower limit on the intrinsic astrophysical scatter in position angles, between the optical and radio bands, of $\sigma_\alpha > 0.212\pi$ radians (or $38.2^{\circ}$) at a $95\%$ confidence level.

==> cleveref/README <==
cleveref, a LaTeX package for intelligent cross-referencing
Copyright (C) 2007--2013  Toby Cubitt

Files:
cleveref.ins  Batch file, run through LaTeX
cleveref.dtx  Docstrip archive, run through LaTeX
cleveref.sty  LaTeX package, generated by cleveref.ins from cleveref.dtx
cleveref.dvi  Package documentation, generated from cleveref.dtx
cleveref.pdf  Package documentation; can also be generated from cleveref.dtx
README        This file

E-mail:   toby-cleveref@dr-qubit.org
Address:  DAMTP, University of Cambridge, United Kingdom

This material is subject to the LaTeX Project Public License. See
http://www.ctan.org/tex-archive/help/Catalogue/licenses.lppl.html for the
details of that license.


Description:
------------
The cleveref package enhances LaTeX's cross-referencing features, allowing the
format of cross-references to be determined automatically according to the
"type" of cross-reference (equation, section, etc.) and the context in which
the cross-reference is used. The formatting for each cross-reference type can
be fully customised in the preamble of your document. In addition, cleveref
can type-set cross-references to lists of multiple labels, automatically
formatting them according to their types, sorting them, and compressing
sequences of numerically consecutive labels. Again, the multiple-reference
formatting is fully customisable. Though a number of other packages provide
similar features, all have certain deficiencies which cleveref attempts to
overcome.

Using cleveref is easy. Basically, wherever you would previously have used
\ref, you can use \cref instead. (Except at the beginning of a sentence, where
you should use \Cref.)  You no longer need to put the name of the thing you're
referencing in front of the \cref command, because cleveref will sort that out
for you: i.e. use "\cref{eq1}" instead of "eq.~(\ref{eq1})". If you want to
refer to a range of labels, use the \crefrange command: "\crefrange{eq1}{eq5}"
produces "eqs.~(1) to~(5)". Finally, if you want to refer to multiple things
at once, you can now combine them all into one cross-reference and leave
cleveref to sort it out: e.g. "\cref{eq2,eq1,eq3,eq5,thm2,def1}" produces:
"eqs.~(1) to~(3) and~(5), theorem~5, and definition~1".

Cleveref has various other useful features. For details, see the package
documentation.

